Reply to Comment on Phys. Rev. Lett. 127, 176601 (2021) by Lee and Yang

In this Reply, we respond to the comments in Phys. Rev. Lett. 130, 219702 (2023) on our Phys. Rev. Lett. 127, 176601 (2021) ''Coulomb instabilities of a three-Dimensional higher-order topological insulator". We show the surface gap given in Phys. Rev. Lett. 130, 219701 (2023) is different from the expression derived by using the well-accepted approach and becomes divergent and singular at lower energies, thus is not suitable for depicting the phase transition from the 2nd-order to 1st-order topological insulator. We further show that a correct surface gap can describe the phase transition if the RG scheme treats the bulk gap as starting point. We justify our criteria in Phys. Rev. Lett. 127, 176601 (2021) for both the transitions from 2nd-order topological insulator to 1st-order topological insulator and normal insulator.

==> author.tex <==


\begin{document}





%\title{Reply to Comment on \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.127.176601}{Phys. Rev. Lett. 127, 176601 (2021)} by Lee and Yang}


\author{Peng-Lu Zhao}
\affiliation{Shenzhen Institute for Quantum Science and Engineering and Department of Physics, Southern University of Science and Technology (SUSTech), Shenzhen 518055, China}
\affiliation{Shenzhen Key Laboratory of Quantum Science and Engineering, Shenzhen 518055, China}

\author{Xiao-Bin Qiang}
\affiliation{Shenzhen Institute for Quantum Science and Engineering and Department of Physics, Southern University of Science and Technology (SUSTech), Shenzhen 518055, China}
\affiliation{Shenzhen Key Laboratory of Quantum Science and Engineering, Shenzhen 518055, China}

\author{Hai-Zhou Lu}
\email{Corresponding author: luhz@sustech.edu.cn}
\affiliation{Shenzhen Institute for Quantum Science and Engineering and Department of Physics, Southern University of Science and Technology (SUSTech), Shenzhen 518055, China}
\affiliation{Shenzhen Key Laboratory of Quantum Science and Engineering, Shenzhen 518055, China}

\author{X. C. Xie}
\affiliation{International Center for Quantum Materials, School of Physics, Peking University, Beijing 100871, China}
\affiliation{CAS Center for Excellence in Topological Quantum Computation, University of Chinese Academy of Sciences, Beijing 100190, China}
\affiliation{Beijing Academy of Quantum Information Sciences, West Building 3, No. 10, Xibeiwang East Road, Haidian District, Beijing 100193, China}



\bibliography{HOTICoul0803}


\end{document}


